The Complexity of Checking Non-Emptiness in Symbolic Tree Automata

We study the satisfiability problem of symbolic tree automata and decompose it into the satisfiability problem of the existential first-order theory of the input characters and the existential monadic second-order theory of the indices of the accepted words. We use our decomposition to obtain tight computational complexity bounds on the decision problem for this automata class and an extension that considers linear arithmetic constraints on the underlying effective Boolean algebra

==> sections/symbolic.tex <==
In this section, we introduce the automata model that we will study in the rest of the paper. Unlike traditional finite automata, symbolic automata read input characters over a not necessarily finite domain, which has the structure of a Boolean algebra of sets defined by a family of monadic predicates. To ensure compatibility with the Boolean algebra operations, the family of monadic predicates defining the sets needs to be closed under propositional operations and contain formulae denoting the empty set and the universe. Furthermore, the definition requires that checking satisfiability of the monadic predicates is decidable. In later sections, we will refine this assumption with different complexity-theoretic bounds.

\begin{definition}[\cite{dantoni_automata_2021}]
\label{def:eba}
An effective Boolean algebra $\mathcal{A}$ is a tuple 
\[
\left(\mathfrak{D}, \Psi, \llbracket \cdot \rrbracket, \perp, \top, \vee, \wedge, \neg\right)
\]
where $\mathfrak{D}$ is a set of domain elements, $\Psi$ is a set of unary predicates over $\mathcal{D}$ that are closed under the Boolean connectives, with $\perp, \top \in \Psi$ and $\llbracket \cdot \rrbracket: \Psi \rightarrow 2^{\mathcal{D}}$ is a function such that \begin{enumerate*}
\item $\llbracket \perp \rrbracket=\emptyset$, 
\item $\llbracket \top \rrbracket=\mathfrak{D}$, and 
\item for all $\psi, \psi_1, \psi_2 \in \Psi$, we have that
\begin{enumerate*}
\item $\llbracket \psi_1 \vee \psi_2 \rrbracket=\llbracket \psi_1 \rrbracket \cup \llbracket \psi_2 \rrbracket$
\item $\llbracket \psi_1 \wedge \psi_2 \rrbracket=\llbracket \psi_1 \rrbracket \cap \llbracket \psi_2 \rrbracket$
\item $\llbracket \lnot \psi \rrbracket=\mathfrak{D} \backslash \llbracket \psi \rrbracket$. 
\end{enumerate*}
\item Checking $\llbracket \psi \rrbracket \neq \emptyset$ is decidable. 
\end{enumerate*} 
A predicate $\psi \in \Psi$ is atomic if it is not a Boolean combination of predicates in $\Psi$. 
\end{definition}

We will give now two examples of the notion of effective Boolean algebra. From the various examples in the literature, we choose one that matches one of our initial motivations: to generalise the complexity results obtained for array theories 
in \cite{alberti_cardinality_2017, raya_vmcai_2022}. We observe that the notion of SMT algebra in \cite[Example~2.3]{dantoni_automata_2021} precisely corresponds to the language introduced in \cite[Definition~5]{raya_vmcai_2022} but omitting cardinality constraints. We take this as a first example of effective Boolean algebra. 

\begin{example} \label{example:smt}
The SMT algebra for a type $\tau$ is the tuple $(\mathcal{D}, \Psi, \llbracket \cdot \rrbracket, \bot, \top, \lor, \land, \lnot)$ where $\mathcal{D}$ is the domain of $\tau$, $\Psi$ is the set of all quantifier-free formulas with one fixed free variable of type $\tau$, $\llbracket \cdot \rrbracket$ maps each monadic predicate to the set of its satisfying assignments, $\bot$ denotes the empty set, $\top$ denotes the universe $\mathcal{D}$ and $\lor, \land, \lnot$ denote the Boolean algebra operations of union, intersection, and complement respectively. 
\end{example}

In applications, it is often useful to consider effective Boolean algebras whose generating monadic predicates use particular representations of formulae. In particular, Example~\ref{example:smt} can be contrasted with other representations of the monadic predicates, which consider implementation details. An example of the latter is the $k$-bit bitvector effective Boolean algebra described in \cite{konstantinidis_applications_2013}.

\begin{example} \label{example:bit}
The powerset algebra $2^{bv(k)}$ is the tuple $(D,\Psi, \llbracket \cdot \rrbracket, \bot, \top, \lor, \land, \lnot)$ where $\mathcal{D}$ is the set $bv(k)$ of all non-negative integers less than $2^k$ or equivalently, all $k$-bit bit-vectors for some $k > 0$, $\Psi$ is the set of BDDs of depth $k$, $\llbracket \cdot \rrbracket$ maps each BDD $\beta$ to the set of all integers $n$ such that the binary representation of $n$ is a solution of $\beta$, $\bot$ denotes the BDD representing the empty set, $\top$ denotes the BDD representing the universal set and $\lor, \land, \lnot$ denote the Boolean algebra operation of union, intersection, and complement as they are implemented for BDDs.
\end{example}

We now introduce the automata model we will investigate in the paper. The crucial difference with traditional finite automata comes in the definition of the transition relation which occurs at two levels: the symbolic level, at which we only consider the particular formula that is satisfied, and the concrete level in which we also consider the input character from the effective Boolean algebra that satisfies the predicate.

\begin{definition}[\cite{dantoni_automata_2021}] \label{def:sfa}
A symbolic finite automaton (s-FA) is a tuple 
\[
M=\left(\mathcal{A}, Q, q_{0}, F, \Delta\right)
\]
where \begin{enumerate*}
\item $\mathcal{A}$ is an effective Boolean algebra.
\item $Q$ is a finite set of states. 
\item $q_{0} \in Q$ is the initial state.
\item $F \subseteq Q$ is the set of final states. 
\item $\Delta \subseteq Q \times \Psi_{\mathcal{A}} \times Q$ is a finite set of transitions.
\end{enumerate*}

A symbolic transition $\rho=\left(q_{1}, \psi, q_{2}\right) \in \Delta$, also denoted $q_{1} \stackrel{\psi}{\rightarrow} q_{2}$, has source state $q_{1}$, target state $q_{2}$, and guard $\psi$. For $d \in \mathfrak{D}$, the concrete transition $q_{1} \stackrel{d}{\rightarrow} q_{2}$ denotes that $q_{1} \stackrel{\psi}{\rightarrow} q_{2}$ and $d \in \llbracket \psi \rrbracket$ for some $\psi$.

A string $w=d_{1} d_{2} \ldots d_{k}$ is accepted at state $q$ if and only if for $1 \leq i \leq k$, there exist transitions $q_{i-1} \stackrel{d_{i}}{\rightarrow} q_{i}$ such that $q_{0}=q$ and $q_{k} \in F$. The set of strings accepted at $q$ is denoted by $\mathcal{L}_{q}(M)$ and the language of $M$ is $\mathcal{L}(M)=\mathcal{L}_{q_0}(M)$.
\end{definition}

We now give examples of automata running over the algebras of Examples~\ref{example:smt} and \ref{example:bit}. We use the traditional graphical representation used in automata theory textbooks \cite{hopcroft_introduction_2006}. As usual, each circle represents a state, the arrows represent the transition relation between states with the corresponding labelling predicate. Final states are denoted by double circle.

\begin{example}[\cite{dantoni_automata_2021}] 
\label{ex:smt-automaton}
We consider the language of linear arithmetic over the integers. We set two formulae $\psi_{> 0}(x) \equiv x > 0$ satisfied by all positive integers and $\psi_{\text{odd}}(x) \equiv x \mod 2 = 1$ satisfied by all odd integers. The following symbolic finite automaton accepts all strings of even length consisting only of positive odd numbers. 


\centering
\begin{tikzpicture} [
    node distance = 3cm, 
    on grid, 
    auto,
    every loop/.style={stealth-}]
 
% State q0 
\node (q0) [state, 
    initial, 
    accepting, 
    initial text = {}] {$q_0$};
 
% State q1    
\node (q1) [state,
    right = of q0] {$q_1$};
 
% Arrows
\path [-stealth, thick]
    (q0) edge[bend left] node {$\psi_{\text{odd}} \land \psi_{> 0}(x)$}   (q1)
    (q1) edge[bend left] node {$\psi_{\text{odd}} \land \psi_{> 0}(x)$}   (q0);
\end{tikzpicture}
\end{example}

\newsavebox{\mydiagram}
\sbox{\mydiagram}{
    \begin{tikzpicture}[node distance=.3cm and .3cm]\footnotesize
    \node (b6) {$b_6$};
    \node (b5) [below right=of b6] {$b_5$};
    \node (b4) [below right=of b5] {$b_4$};
    \node (b3) [below right=of b4] {$b_3$};
    \node (b2) [below left=of b3] {$b_2$};
    \node (b1) [below=of b2] {$b_1$};
    \node (top) [below right=of b1] {$\top$};
    \node (bot) [below left=of b1] {$\bot$};

    \draw[zeroarrow] (b6) -- (b5);
    \draw[zeroarrow] (b6) -- (b5);
    \draw[onearrow] (b5) -- (b4);
    \draw[onearrow] (b4) -- (b3);
    \draw[onearrow] (b3) -- (b2);
    \draw[zeroarrow] (b2) -- (b1);
    \draw[zeroarrow] (b1) -- (top);
    \draw[zeroarrow] (b3) -- (top);
    \draw[onearrow] (b2) -- (bot);
    \draw[onearrow] (b6) -- (bot);
    \draw[zeroarrow] (b5) -- (bot);
    \draw[zeroarrow] (b4) -- (bot);

    \end{tikzpicture}
}

\begin{example}[\cite{konstantinidis_applications_2013}]
We consider the language of BDDs over bit-vectors of length six. The following symbolic finite automaton accepts all strings that start by a bit-vector representing either of the numbers $6,14,22,38$ or $54$ followed by an arbitrary number of bit-vectors.

\centering
\begin{tikzpicture} [
    node distance = 5cm, 
    on grid, 
    auto,
    every loop/.style={stealth-}]
 
% State q0 
\node (q0) [state, 
    initial, 
    initial text = {}] {$q_0$};
 
% State q1    
\node (q1) [state,
    accepting,
    right = of q0] {$q_1$};
 
% Arrows
\path [-stealth, thick]
    (q0) edge node {\usebox{\mydiagram}}   (q1)
    (q1) edge [loop above]  node {$\top$}();
\end{tikzpicture}
\end{example}




